What's Different between Visual Question Answering for Machine "Understanding" Versus for Accessibility?

In visual question answering (VQA), a machine must answer a question given an associated image. Recently, accessibility researchers have explored whether VQA can be deployed in a real-world setting where users with visual impairments learn about their environment by capturing their visual surroundings and asking questions. However, most of the existing benchmarking datasets for VQA focus on machine "understanding" and it remains unclear how progress on those datasets corresponds to improvements in this real-world use case. We aim to answer this question by evaluating discrepancies between machine "understanding" datasets (VQA-v2) and accessibility datasets (VizWiz) by evaluating a variety of VQA models. Based on our findings, we discuss opportunities and challenges in VQA for accessibility and suggest directions for future work.

==> tex/finding2.tex <==

\subsection{Model Performance}
First, we examine whether the progress of VQA models on the ``machine understanding'' dataset (VQA-v2) also apply to the accessibility dataset (VizWiz).
We thus pick six models from 2015 to 2021 on the VQA-v2 leaderboard and evaluate them on both the VQA-v2 and VizWiz datasets. 
For VizWiz, we report testing results on both trained from scratch with VizWiz and trained on VQA-v2 and finetuned with VizWiz. See appendix for implementation details. 

% First of all, we assess model performances on the VizWiz dataset by looking into two research questions: 1) how well do the VQA models perform on the VizWiz dataset comparing to the VQA-v2 benchmark dataset and 2) whether the model advancements on the VQA-v2 dataset actually improve the model performance on the VizWiz dataset. 

% To answer these question, we pick five models from 2015 to 2019, including the state-of-art VQA model Pythia. We introduced the models in section 3. 
% We test these models on both the VQA-v2 and the VizWiz datasets. For VizWiz, we finetune the models on VizWiz before testing. See appendix for implementation details. 

The results are shown in \autoref{tab:model-performance}. 
We also show performance improvement based on question types. Results are in figure TODO.
We see that the model advancements on VQA-v2 also apply to the VizWiz dataset. This indicates works that improve the VQA-v2 benchmark are beneficial in real-life application that assists visually-impaired people.  
However, we also find significant gaps of model performance between the two datasets. The best model for VizWiz has accuracy score $51.4$ (from Pythia), which is still significantly lower than the MFB model's score on VQA-v2 in 2015 (with score gap of $14$). Meanwhile, model performance on VQA-v2 only improved around $3$ from 2015 to 2019. 

A possible reason of the significant score gap is the training dataset size difference. 
VizWiz dataset includes around $32,000$ image and question pairs whereas VQA-v2 includes around $1,000,000$ image and question pairs. 
Thus, to perform a fair comparison, we re-train the models on a random subset of VQA-v2 dataset to match the size of the VizWiz dataset.
Table todo shows the results. 
(Hopefully) we see that though the small VQA-v2 performance is lower than the original VQA-v2 score, it is still significantly higher than the model performance on VizWiz dataset. 

Overall, this shows that it is non-trivial to adapt models that were developed focusing on ``machine understaning'' to real-life applications as real-life data can be very different from crowdsourced synthetic data. 
% which is reasonable as VizWiz samples data from real-life situations while VQA-v2 is a crowdsourced dataset. 
% This suggests that in order to really help the people with visual impairments, the field should work on the real data from visually-impaired people rather than chasing leaderboards.  



\subsection{Error Analysis on Data Discrepancies}
To better adapt the VQA model on the VizWiz dataset, we then want to understand how does the VizWiz dataset differ from the VQA-v2 dataset and how does the differences affect model performance. 
We thus conduct an error analysis on the best performed model ALBEF with the following research questions.
We perform the analysis on the VizWiz validation dataset and a random subset of the VQA-v2 validation dataset to match the size of the VizWiz dataset. 

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{heat map.png}
    \caption{The ALBEF model accuracy based on data point's likelihood of being a VizWiz data. (note should do reverse -- likelihood of being VQA data).}
    \label{fig:heatmap}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{prob.png}
    \caption{The ALBEF model accuracy based on data point's likelihood of being a VizWiz data for each question type. (note should do reverse -- likelihood of being VQA data).}
    \label{fig:avg_prob}
\end{figure}

\paragraph{Q1: Does model perform better on data more similar to VQA-v2 data?\\}
Since ALBEF model has significantly higher accuracy score on the VQA-v2 dataset comparing to the VizWiz dataset, we want to validate whether the performance gap is caused by the dataset discrepancy. 
We thus train a image discriminator and a question discriminator to distinguish whether the data point image or question is from VizWiz as oppose to from VQA-v2 using the training data from each dataset.
Both of the discriminators have high accuracy $todo$.
The discriminator's confidence score of the data point belonging to VizWiz then is used to indicate how similar is the VizWiz data point to VQA-v2 data. 
We answer the experiment question by assessing the correlation between the model performance and the similarity score from the discriminator on the VizWiz validation dataset. 


Results are in \autoref{fig:heatmap}.
We also look into each question type... Results are shown in \autoref{fig:avg_prob}

We also look into $50-100$ data points that have high similarity score but low performance and low similarity and performance scores. We find ... pattern.

\begin{figure*}[h]
    \centering
    \includegraphics[width=2\columnwidth]{qcluster.png}
    \caption{Model performance distribution of the two datasets based on question clustering.}
    \label{fig:q_cluster}
\end{figure*}

\paragraph{Q2: Which part of the data contribute more to the low performance, questions or images?\\}
For future model or dataset improvement, we investigate whether it is the discrepancy of questions or images of the two dataset causing the performance gap. 
In order to quantify the effect of image discrepancies on the model performance, we need to disentangle the image effect from the question effect.
Therefore, we first cluster the VQA and VizWiz validation data points by their questions into $100$ clusters using K-nearest neighbor algorithm. 
Then, we compute the distributions of ALBEF model performance on both datasets over the clusters. 
Finally, the distribution difference represents the performance gap caused by image discrepancies of the two datasets.
Same apply to the question discrepancies. 


\ shows the score distribution of two datasets clustered by questions. Thus the distribution gap represents the performance gap caused by image discrepancies. We estimate the distribution gap by averaging the score differences of each question cluster. Here is distribution gap is $todo$.
Similarly, fig todo shows the two distributions clustered by images. From this result, the distribution gap caused by question discrepancies is $todo$.
It indicates that future work should ... (pay more attention to the image/questions?).

\paragraph{Q3: For both the question and image, what type of data requires more attention to improve model performance?\\}
Finally, we look into the distribution differences between the two datasets and figure out what type of data points are difficult for the model. 
We look into clusters where both dataset distribution has low performance on.
They are ...

We also look into clusters where the model perform well on VQA but not on VizWiz.
We first compute TSNE score for the VQA-v2 and VizWiz validation data on both image and questions. 
Then within each of these clusters, we look into the image/question distribution through TSNE and find. 


\subsection{Discussion}



